Making sense of sensory input

This paper attempts to answer a central question in unsupervised learning: what does it mean to "make sense" of a sensory sequence? In our formalization, making sense involves constructing a symbolic causal theory that both explains the sensory sequence and also satisfies a set of unity conditions. The unity conditions insist that the constituents of the causal theory -- objects, properties, and laws -- must be integrated into a coherent whole. On our account, making sense of sensory input is a type of program synthesis, but it is unsupervised program synthesis. Our second contribution is a computer implementation, the Apperception Engine, that was designed to satisfy the above requirements. Our system is able to produce interpretable human-readable causal theories from very small amounts of data, because of the strong inductive bias provided by the unity conditions. A causal theory produced by our system is able to predict future sensor readings, as well as retrodict earlier readings, and impute (fill in the blanks of) missing sensory readings, in any combination. We tested the engine in a diverse variety of domains, including cellular automata, rhythms and simple nursery tunes, multi-modal binding problems, occlusion tasks, and sequence induction intelligence tests. In each domain, we test our engine's ability to predict future sensor values, retrodict earlier sensor values, and impute missing sensory data. The engine performs well in all these domains, significantly out-performing neural net baselines. We note in particular that in the sequence induction intelligence tests, our system achieved human-level performance. This is notable because our system is not a bespoke system designed specifically to solve intelligence tests, but a general-purpose system that was designed to make sense of any sensory sequence.

==> tex/discrete-conclusion.tex <==


\section{Discussion}
\label{sec:conclusion}

This chapter is an attempt to answer a key question of unsupervised learning: what does it mean to ``make sense'' of a (discretised) sensory sequence? 
Our answer is broadly Kantian \cite{chalmers1992high}: making sense means positing a collection of objects that persist over time, with attributes that change over time, according to intelligible laws.
As well as providing a precise formalization of this task, we also provide a concrete implementation of a system that is able to make sense of the sensory stream.
We have tested the \sys{} in a variety of domains;
in each domain, we tested its ability to predict future values, retrodict previous values, and impute missing intermediate values. 
Our system achieves good results across the board.

Of particular note is that it is able to achieve human performance on challenging sequence induction IQ tasks.
We stress, once more, that the system was not hard-coded to solve these tasks.
Rather, it is a general \emph{domain-independent} sense-making system that is able to apply its general architecture to the particular problem of Seek Whence induction tasks, and is able to solve these problems ``out of the box'' without human hand-engineered help.
We also stress, again, that the system did not learn to solve these sequence induction tasks by being presented with hundreds of training examples\footnote{
Raven's progressive matrices \cite{carpenter1990one}  are spatial reasoning tasks requiring inductive reasoning. 
Barrett et al \cite{barrett2018measuring} train a neural network to learn to solve Raven's progressive matrices, but their method requires millions of training examples.}. 
Indeed, the system had never seen a \emph{single} such task before.
Instead, it applied its general sense-making urge to each individual task, \emph{de novo}.
We also stress that the interpretations produced are human readable and can be used to provide explanations and justifications of the decisions taken:
when the \sys{} produces an interpretation, we can not only see what it predicts will happen next, but we can also understand \emph{why} it thinks this is the right continuation. 
We believe these results are highly suggestive, and shows that a sense-making component such as this will be a key aspect of any general intelligence.
%We do not claim, of course, that any such sense-making machine must have the same precise architecture as that described in Section \ref{sec:system}. But we \emph{do} claim that it must satisfy the conditions of sense-making of Definition \ref{def:apperception-task}. 

Our architecture, an unsupervised program synthesis system, is a purely symbolic system, and 
as such, it inherits two key advantages of ILP systems \cite{evans2018learning}.
First, the interpretations produced are \emph{interpretable}. 
Because the output is symbolic, it can be read and verified by a human\footnote{Large machine-generated programs are not always easy to understand. But machine-generated symbolic programs are certainly easier to understand than the weights of a neural network. See Muggleton et al \cite{muggleton2018ultra} for an extensive discussion. }.
Second, it is very \emph{data-efficient}.
Because of the language bias of the \logic{} language, and the strong inductive bias provided by the Kantian unity conditions, the system is able to make sense of extremely short sequences of sensory data, without having seen any others.
%The reason for this data-efficiency is the language bias preferring short programs over longer ones: a short general program will be preferred to a larger program consisting of many special-case ad-hoc rules that happen to cover the input sequence.
%A third key advantage of symbolic program synthesis methods is that they support continual learning as solutions learned in one task can be reused in the next to reduce the search-space\cite{lin2014bias}.

However, the system in its current form has some clear limitations.
First, it does not currently handle noise in the sensory input.
All sensory information is assumed to be significant, and the system will strive to find an explanation of \emph{every} sensor reading.
There is no room for the idea that some sensor readings are inaccurate.

Second, the sensory input must be discretized before it can be passed to the system.
We assume some prior system has already discretized the continuous sensory values by grouping them into classes.

The first limitation is addressed in Section \ref{sec:noise}, and the second limitation is addressed in Chapter \ref{chapter:making-sense-raw}.



==> tex/discrete-house.tex <==
\section{Experiment 2: the house}
\label{sec:house}

In the \emph{Second Analogy}, Kant describes the following example:
\begin{quote}
The apprehension of the manifold of appearance is always successive. The representations of the parts succeed one another. Whether they also succeed in the object is a second point for reflection, which is not contained in the first... Thus, e.g., the apprehension of the manifold in the appearance of a house that stands before me is successive. Now the question is whether the manifold of this house itself is also successive, which certainly no one will concede. [A189/B234ff] 
\end{quote}
Here, Kant asks us to imagine an agent surveying a large house from close range. Its visual field cannot take in the whole house in one glance, so its focus moves from one part of the house to another.
Its sequence of visual impressions is successive, but there is a further question whether a pair of (subjectively) successive visual impressions represents the house at a single moment of objective time, or at two successive moments of objective time.

In the B edition of the \emph{Transcendental Deduction}, Kant contrasts the example of the house with another example: an agent watching water slowly freeze:
\begin{quote}
Thus if, e.g., I make the empirical intuition of a house into perception through apprehension of its manifold, my ground is the necessary unity of space and of outer sensible intuition in general, and I as it were draw its shape in agreement with this synthetic unity of the manifold in space...
If (in another example) I perceive the freezing of water, I apprehend two states (of fluidity and solidity) as ones standing in a relation of time to each other.
[B162]
\end{quote}
Kant asks us to compare and contrast the two cases of subjective succession. 
In the first case, the subjective succession represents an \emph{objective simultaneity}: the perceived state of the top of the house is simultaneous with the perceived state of the bottom of the house, even if the subjective impressions are successive. 
In the second case, by contrast, the subjective succession represents an \emph{objective succession}: the water's transition from liquid to solid is a fact about the world, not just about my mental states. 
Kant characterises the difference between the two cases in terms of modality: in the case of the house, I could have received the impressions in a different order: I could have seen the bottom of the house before the top. But in the case of the water freezing, I could not have seen the solid state before the liquid state.\footnote{See \cite[p.358]{longuenesse1998kant}.}

We gave the \sys{} a simplified version of Kant's example (see Figure \ref{fig:house-1}).
In our experiment, there is a pixel image that is too large for the agent to survey in one glance. 
The agent's sensors are only able to take in a small window of the image at any moment, and the agent must move the sensory window around to survey the whole image. 
Just as in Kant's case, where we cannot take in the whole of the house in one glance, here the agent cannot take in the whole of the pixel image at one glance,  and must reconstruct it from the succession of fragments. 

Note that in this experiment, the actions are exogenous and do not need to be explained by the \sys{}.
What does need to be explained is the changing sensor information.

When we give the sequence of Figure \ref{fig:house-1} to the \sys{}, it is able to reconstruct the complete picture from the sequence of incomplete partial perceptions.
The best theory it finds is $\theta = (\phi, I, R, C)$ where:
\begin{eqnarray*}
I & = & \bigsetbegin{} 
\begin{tabular}{llll}
$\mathit{off}(w_{1,2})$ &
$\mathit{off}(w_{1,3})$ &
$\mathit{off}(w_{2,3})$ &
$\mathit{off}(w_{3,2})$ \\
$\mathit{off}(w_{4,2})$ &
$\mathit{off}(w_{4,3})$ &
$\mathit{on}(w_{1,1})$ &
$\mathit{on}(w_{1,4})$ \\
$\mathit{on}(w_{2,1})$ &
$\mathit{on}(w_{2,2})$ &
$\mathit{on}(w_{2,4})$ &
$\mathit{on}(w_{3,1})$ \\
$\mathit{on}(w_{3,3})$ &
$\mathit{on}(w_{3,4})$ &
$\mathit{on}(w_{4,1})$ &
$\mathit{on}(w_{4,4})$ \\
$\mathit{in}(v_{1,1}, w_{1,4})$ &
$\mathit{in}(v_{1,2}, w_{1,3})$ &
$\mathit{in}(v_{2,1}, w_{2,4})$ &
$\mathit{in}(v_{2,2}, w_{2,3})$
\end{tabular}
\bigsetend{} \\
R & = & \bigsetbegin{} 
\mathit{off}(W) \wedge \mathit{in}(V, W) \wedge \mathit{zero}(N) \rightarrow \mathit{intensity}(V, N) \\
\mathit{on}(W) \wedge \mathit{in}(V, W) \wedge \mathit{one}(N) \rightarrow \mathit{intensity}(V, N) \\
\mathit{right}(M) \wedge r(W, W_2) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{left}(M) \wedge r(W_2, W) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{up}(M) \wedge b(W, W_2) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{down}(M) \wedge b(W_2, W) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2)
\bigsetend{} \\
C & = & \bigsetbegin{}
\forall C{:}\mathit{cell}, \mathit{on}(X) \oplus \mathit{off}(X) \\
\forall V{:}\mathit{sensor}, \exists ! C{:}\mathit{cell}, \mathit{in}(V, C) \\
\forall V{:}\mathit{sensor}, \exists ! N{:}\mathit{number}, \mathit{intensity}(C, N)
\bigsetend{}
\end{eqnarray*}
Here, the initial conditions $I$ specify the on/off values of the sixteen pixels $\{w_{i,j} \mid i \in \{1..4\}, j \in \{1..4\}\}$, and the initial placements of the four sensors $\{v_{i,j} \mid i \in \{1,2\}, j \in \{1,2\}\}$.
Note that the on/off values of the  pixels do not change over time. 
The 2D spatial relations between the cells $w_{i,j}$ are represented by the $r$ and $b$ relations. E.g. $r(w_{1,1}, w_{2,1})$, $b(w_{1,1}, w_{1,2})$. The spatial relations using $r$ and $b$ are provided as background knowledge.

The first two rules state that if a sensor is attached to a cell, and that cell is on (respectively off), then the intensity of the sensory is 1 (respectively 0).
The other rules describe how the sensors move as the actions are performed.
Note that the image reconstructed by the \sys{} is a mirror image of the original image used to generate the sensory data.
Figure \ref{fig:house-2}(b) shows the sequence as reconstructed by the \sys{}.
In this interpretation, the original image has been flipped vertically, and the actions ``up'' and ``down'' have been interpreted as ``down'' and ``up'' respectively.


\begin{figure}
\centering
\includegraphics[scale=0.4]{figs/kant/house-full.pdf}
\caption[The sensory sequence for the ``house'' example]{For each of the sixteen time-steps, we show the $4 \times 4$ pixel grid and the positions of the sensors (as a red square), the action performed, and the values of the four sensors. }
\label{fig:house-1}
\end{figure}


\begin{figure}
\centering
\begin{minipage}{13 cm}
  \subfloat[]{%
    \makebox[\textwidth][c]{\includegraphics[scale=0.4]{figs/kant/house1.pdf}}
  }
  \\
  \subfloat[]{%
    \makebox[\textwidth][c]{\includegraphics[scale=0.4]{figs/kant/house2.pdf}}
  }  
\caption[Comparing the ground truth with the engine's reconstruction]{The top row (a) shows the ground truth used to generate the sensory data, while the bottom row (b) shows the reconstruction made by the \sys{}. Note that the reconstruction is a mirror image of the ground truth, flipped vertically, in which ``up'' is interpreted as down, and ``down'' is interpreted as up. }
\label{fig:house-2}
\end{minipage}
\end{figure}

Thus, the \sys{} is able to make sense of Kant's famous ``house'' example [B162]:
the engine posits a two-dimensional array of pixels and interprets the sensors as moving across the array.
Although the sensory readings are successive, the engine posits an \emph{objective simultaneity} to explain the subjective succession of sensor readings. % For example, the pixel at (1,1) being on is simultaneous with the pixel at (1,2) being off.


